Predicting Stable Configurations for Semantic Placement of Novel Objects

Human environments contain numerous objects configured in a variety of arrangements. Our goal is to enable robots to repose previously unseen objects according to learned semantic relationships in novel environments. We break this problem down into two parts: (1) finding physically valid locations for the objects and (2) determining if those poses satisfy learned, high-level semantic relationships. We build our models and training from the ground up to be tightly integrated with our proposed planning algorithm for semantic placement of unknown objects. We train our models purely in simulation, with no fine-tuning needed for use in the real world. Our approach enables motion planning for semantic rearrangement of unknown objects in scenes with varying geometry from only RGB-D sensing. Our experiments through a set of simulated ablations demonstrate that using a relational classifier alone is not sufficient for reliable planning. We further demonstrate the ability of our planner to generate and execute diverse manipulation plans through a set of real-world experiments with a variety of objects.

==> 03background.tex <==
%Mees et al.~\cite{mees2020learning} look at learning language relationships between different %objects on RGB images.  used an MCTS-based approach to dinf 
%Key difference: language, RGB images, no unknown objects.

% \textbf{Relational learning.}
% https://arxiv.org/pdf/2012.13693.pdf
\textbf{Learning relations.}
Semantic relations are important to teaching and instructing robot tasks~\cite{forbes2015robot}.
\citet{paul2016efficient} look at efficient grounding of spatial information in a way that supports complex multi-object relationships, but mostly look at simple objects and do not look at grounding from raw perception data. They also mostly look at identifying \textit{specific} objects that fit a complex statement; we look at placement in free space, where objects might meet various conditions.
Other work has specifically looked at modeling relationships between objects. \citet{venkatesh2020spatial} look at learning language-grounded spatial relationships. 
% https://arxiv.org/pdf/2012.08508.pdf
\citet{ding2020object} use a distributional approach instead of neural-symbolic approaches to learn object relational models.
\citet{rosman2011learning} classify simple predicates of pairs of objects by utilizing features from contact-based relationships.
\citet{mees2020learning} learn spatial distributions of feasible object locations on a tabletop, but don't look at generalization to the camera frame in the same way we do, and do not use unknown objects.
It also increasingly seems that graph-based representations are a strong way of encoding the relationships between objects; for example, \citet{bear2020learning} have looked at learning graph neural net representations of whole scenes, while \citet{wilson-corl2019-collection-pushing} learn to rearrange collections of objects into group piles via pushing. This work is complementary to ours.
Recently, \citet{sharma2020relational} specifically looked at learning relational models for skill preconditions.
%Implicitly, much language-based work must learn these sorts oations; e.g. 

\textbf{Task planning using learned models.} 
A number of recent approaches have looked at learning for longer-horizon manipulation tasks. 
Regression Planning Networks~\cite{xu2019regression} have to learn dependencies between objects and compute action preconditions. \citet{huang2019continuous} learned precondition networks for different objects based on continuous state, using a relaxation for task planning.
Visual Robot Task Planning~\cite{paxton2019visual} used an MCTS-based approach to find plans to complete a simple stacking task.
Deep Planning Domain Learning~\cite{kase2020transferable} looked at learning sets of predicates which could be used by a task planner, but don't use these for planning placements or determining the next action, instead learning a separate model-free low level policy for execution.
In other recent work, Simeonov et al~\cite{simeonov2020long} propose a long-horizon planning system for rigid point cloud objects,
but they look specifically at multi-step planning where the high level task is given and do not look at cluttered scenes or consider changing scene geometry. We look at a subset of this problem, focusing on learning models of relationships that might fit into task planning.

Another way of looking at complex manipulation tasks is to learn more model-free neural net policies instead of explicit models of conditions and effects.
Neural Task Graphs~\cite{huang-cvpr2019-ntg}, for example, estimate the current state for complex tasks given a single demonstration. 
Deep Affordance Foresight~\cite{xu2020deep} looks at predicting sequences of possible actions to accomplish long horizon tasks, but isn't necessarily looking at generalizing across objects or geometry.


\textbf{Grasping.} 
There is a large variety of learning-based grasp planners~\cite{saxena2006learning,lenz2015deep,mahler2016dexnet,lu2017grasp,mousavian20196,lu2020multi,liu2019generating} available that could be used as a part of our planner.
Our approach fits within the recently popular optimization-based grasp planning paradigm, leveraging neural network classifiers for grasp success detection~\cite{mousavian20196,lu2017grasp,liu2019generating,lu2020multi}. Most closely related is the approach of Lu et al.~\cite{lu2020multi} that uses a voxel-based representation with an MDN prior to predict grasp success; this can be seen as a particular subset of the predicate learning problem addressed in this paper. We specifically use 6-DOF GraspNet~\cite{mousavian20196} to generate grasps to test our method on the real system, because it generates a large number of very reliable grasps for a wide range of objects.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "00main"
%%% End:


==> 91extra.tex <==
\begin{table*}[h]
\centering
 \begin{tabular}{l p{4cm} p{4cm}}
 \hline
 Tabletop & Kitchen & Notes\\ \hline
 is\_aligned(o1, o2) & gripper\_is\_aligned & Definition depends a lot on the objects.\\
 left\_of(o1, o2) & & just a dimension check for a particular axis (x axis)\\
 right\_of(o1, o2) & & same (x axis)\\
 in\_front\_of(o1, o2) & & same (z axis)\\
 behind(o1, o2) & & same (z axis)\\
 over(o1, o2) & & same (y axis)\\
 below(o1, o2) & & same (y axis)\\
 is\_occluded(o1, o2) & & Is o1 occluded by o2?\\
 inside\_of(o1, o2) & & How do we implement this? probably distance to a couple points\\
 around(o1, o2) & around\_handle, around\_rim, \dots & \\
 free\_of & & Basically inverse of around? \\
 stable\_placement(o1, surface) & & \\
 canonical\_placement(o1, surface) & & \\
 near(o1, o2) & & Would be interesting if this were a ternary relation. E.g. o1 is near o2 if o3 is further away\\
 far(o1, o2) & & Would be interesting if this were a ternary relation \\
 \hline
\end{tabular}
\caption{Predicates for experimental setups}
\label{table:predicates}
\end{table*}


This is a diagram of the diffetrent predicates from Chris Xie
